Faster Post-Quantum TLS 1.3 Based on ML-KEM: Implementation and Assessment

TLS is extensively utilized for secure data transmission over networks. However, with the advent of quantum computers, the security of TLS based on traditional public-key cryptography is under threat. To counter quantum threats, it is imperative to integrate post-quantum algorithms into TLS. Most PQ-TLS research focuses on integration and evaluation, but few studies address the improvement of PQ-TLS performance by optimizing PQC implementation. For the TLS protocol, handshake performance is crucial, and for post-quantum TLS (PQ-TLS) the performance of post-quantum key encapsulation mechanisms (KEMs) directly impacts handshake performance. In this work, we explore the impact of post-quantum KEMs on PQ-TLS performance. We explore how to improve ML-KEM performance using the latest Intel's Advanced Vector Extensions instruction set AVX-512. We detail a spectrum of techniques devised to parallelize polynomial multiplication, modular reduction, and other computationally intensive modules within ML-KEM. Our optimized ML-KEM implementation achieves up to 1.64x speedup compared to the latest AVX2 implementation. Furthermore, we introduce a novel batch key generation method for ML-KEM that can seamlessly integrate into the TLS protocols. The batch method accelerates the key generation procedure by 3.5x to 4.9x. We integrate the optimized AVX-512 implementation of ML-KEM into TLS 1.3, and assess handshake performance under both PQ-only and hybrid modes. The assessment demonstrates that our faster ML-KEM implementation results in a higher number of TLS 1.3 handshakes per second under both modes. Additionally, we revisit two IND-1-CCA KEM constructions discussed in Eurocrypt22 and Asiacrypt23. Besides, we implement them based on ML-KEM and integrate the one of better performance into TLS 1.3 with benchmarks.

==> Algorithms/barrett.tex <==
\begin{algorithm}[htbp]
  \caption{Signed Barrett reduction \cite{DBLP:journals/iacr/Seiler18}}
  \label{algo:barrettreduction}
  \small
  \begin{algorithmic}[1]
    \Require Signed integer $a$ where $-\beta / 2 \leq a<\beta/ 2$ and $q < \beta / 2$. 
    \Ensure Signed integer $r \equiv a(\bmod q)$ where $0 \leq r\leq q$.
    \State $v \leftarrow\left\lfloor\frac{2^{\lfloor\log (q)\rfloor-1} \beta}{q}\right\rceil$
    \State $t \leftarrow\left\lfloor\frac{a v}{2^{\lfloor\log (q)\rfloor-1} \beta}\right\rfloor$
    \State $r \leftarrow a-(t q \bmod \beta)$
    \State \textbf{Return} $r$
  \end{algorithmic}
\end{algorithm}


==> Algorithms/montgomery.tex <==
\begin{algorithm}[htbp]
  \caption{Signed Montgomery reduction \cite{DBLP:journals/iacr/Seiler18}}
  \label{algo:montreduction}
  \small
  \begin{algorithmic}[1]
    \Require Signed integer $a=a_1 \beta+a_0$ where $-\beta q / 2 \leq a<\beta q / 2$ and $0 \leq a_0<\beta$. 
    \Ensure Signed integer $r^{\prime} \equiv \beta^{-1} a(\bmod q)$ where $-q<r^{\prime}<q$.
    \State $m \leftarrow a_0 q^{-1} \bmod ^{ \pm} \beta$
    \State $t_1 \leftarrow\left\lfloor m \cdot \frac{q}{\beta}\right\rfloor$
    \State $\mathrm{r}^{\prime} \leftarrow a_1-t_1$
    \State \textbf{Return} $r'$
  \end{algorithmic}
\end{algorithm}


==> Tables/MLDSAparameters.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
% \begin{tabular}{c|c|c|c|c|c|c|c}
% \toprule
%           &     &      &   &   &   &    &   \\ \midrule
% KYBER512  & 256 & 3329 & 2 & 3 & 2 & 10 & 4 \\
% KYBER768  & 256 & 3329 & 3 & 2 & 2 & 10 & 4 \\
% KYBER1024 & 256 & 3329 & 4 & 2 & 2 & 11 & 5 \\ \bottomrule
% \end{tabular}
% \label{tab:ML-KEMpar}
% \end{table}


\begin{table}
	\centering
	\fontsize{8}{10}\selectfont    %{字体尺寸}{行距}
        \tabcolsep=0.2cm
	\caption{ML-DSA parameter sets.}
	\begin{tabular}{c|cccccccccc}
		\toprule
		Scheme  & $q$ & $d$ & $\tau$ & $\lambda$ & $\gamma_1$ & $\gamma_2$ & $(k,l)$ & $\eta$& $\beta$ & $\omega$\\
		\hline
		ML-DSA-44  & 8380417 & 13 & 39 & 128 & $2^{17}$ &$(q-1)/88$ & (4,4) &2 & 78 &80  \\
		ML-DSA-65 & 8380417 & 13 & 49 & 192 & $2^{19}$ &$(q-1)/32$ & (6,5) &4 & 196 &55\\
		ML-DSA-87  & 8380417 & 13 & 60 & 256 & $2^{19}$ &$(q-1)/32$ & (8,7) &2 & 120 &75   \\
		\bottomrule
	\end{tabular}\vspace{0cm}
	\label{tab:ML-KEMpar}
\end{table}


==> Tables/MLKEMparameters.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
% \begin{tabular}{c|c|c|c|c|c|c|c}
% \toprule
%           &     &      &   &   &   &    &   \\ \midrule
% KYBER512  & 256 & 3329 & 2 & 3 & 2 & 10 & 4 \\
% KYBER768  & 256 & 3329 & 3 & 2 & 2 & 10 & 4 \\
% KYBER1024 & 256 & 3329 & 4 & 2 & 2 & 11 & 5 \\ \bottomrule
% \end{tabular}
% \label{tab:ML-KEMpar}
% \end{table}


\begin{table}
        \fontsize{6.5}{8}\selectfont 
	\centering
        \tabcolsep=0.35cm
	\caption{ML-KEM parameter sets.}
	\begin{tabular}{c|ccccccc}
		\toprule
		Scheme  & $n$ & $q$ & $k$ & $\eta_1$ & $\eta_2$ & $d_u$ & $d_v$ \\
		\hline
		ML-KEM-512  & 256 & 3329 & 2 & 3 & 2 & 10 & 4  \\
		ML-KEM-768& 256 & 3329 & 3 & 2 & 2 & 10 & 4\\
		ML-KEM-1024  & 256 & 3329 & 4 & 2 & 2 & 11 & 5   \\
		\bottomrule
	\end{tabular}\vspace{0cm}
	\label{tab:ML-KEMpar}
\end{table}

